Pretrained Embeddings for E-commerce Machine Learning: When it Fails and Why?

The use of pretrained embeddings has become widespread in modern e-commerce machine learning (ML) systems. In practice, however, we have encountered several key issues when using pretrained embedding in a real-world production system, many of which cannot be fully explained by current knowledge. Unfortunately, we find that there is a lack of a thorough understanding of how pre-trained embeddings work, especially their intrinsic properties and interactions with downstream tasks. Consequently, it becomes challenging to make interactive and scalable decisions regarding the use of pre-trained embeddings in practice. Our investigation leads to two significant discoveries about using pretrained embeddings in e-commerce applications. Firstly, we find that the design of the pretraining and downstream models, particularly how they encode and decode information via embedding vectors, can have a profound impact. Secondly, we establish a principled perspective of pre-trained embeddings via the lens of kernel analysis, which can be used to evaluate their predictability, interactively and scalably. These findings help to address the practical challenges we faced and offer valuable guidance for successful adoption of pretrained embeddings in real-world production. Our conclusions are backed by solid theoretical reasoning, benchmark experiments, as well as online testings.

==> experiment.tex <==
The goal of the experiments is to justify the major claims and theoretical results in our paper. All the reported results are averaged from five independent runs, the implementation code and data links are also provided in the online material. 

\subsection{Data set, preprocessing and task settings}
\label{sec:data}

We use benchmark datasets for illustration and reproducibility purposes. We rely on the production platform of \emph{Walmart.com} to carry online experiments. The three benchmark datasets are summarized as follow:
\begin{itemize}
    \item \textbf{MovieLens-1M}: the MovieLens dataset collects the users' ratings of the movies. It consists of around 1 million ratings from 6,040 users on 3,925 movies. The dataset has been preprocessed, and we covert the rating to implicit feedback (interacted or not). Each movie has the title information and the genre categorization. 
    \item \textbf{Instacart}: the Instacart data collect the online grocery baskets, and consists of $\sim$3 million orders from around 50,000 products and 200,000 users. Each grocery item has the title information and the aisle (category) of the item.
    \item \textbf{Amazon Electronics}: the dataset collects $\sim$1 million reviews from the customers who have purchased electronic products from Amazon. It consists of around 60,000 items and 200 thousand users. The metadata includes item titles and their category hierarchy.
\end{itemize}
For preprocessing, we remove items and users with less than five interactions for the Instacart and Amazon dataset to match with the proprocessed MovieLens data. When training Dov2vec \cite{le2014distributed}, the titles of the movie and products are tokenized using the \emph{Gensim} python library\footnote{\url{https://radimrehurek.com/gensim/parsing/preprocessing.html}}. When using the BERT model for title embedding \cite{devlin2018bert}, the preprocessing uses the official BERT pipeline\footnote{\url{https://www.tensorflow.org/official_models/fine_tuning_bert}}.

We design two types of tasks: item (movie) classification and sequential recommendation tasks. The item classifications will be introduced later according to the context. For the sequential recommendation tasks, we adopt the training, validation and evaluation setup introduced in \cite{kang2018self}. 


\subsection{Results and analysis}
\label{sec:result}

\textbf{Model design for i.i.d downstream generalization}. We first justify our theoretical results in Section \ref{sec:structure}. To construct the i.i.d environment for CL-based pre-training, for each item $x$, we sample $x^+$ from the same category (or genre), and $x^-$ is drawn randomly. The downstream task is item classification. Here, we strictly recovers the setting in Section \ref{sec:structure} because the environment does change from pre-training to downstream task. In downstream task, we use the embeddings as input and train the model on 80\% of the items with their labels (if needed). For the same-structure pre-training, we use BERT that takes the tokenized item titles as input, also fine tune it on 80\% of the items, and extract the last layer as remaining items' embedding for testing i.i.d generalization. We use two types of downstream model structure: a linear regression (\textbf{LR}) model (already included in BERT during fine-tuning), and inner product (\textbf{IP}). We use such as \textbf{CL-LR} to denote the combination. The results are provided in Table \ref{tab:offline_eval}. We see that the best performances are achieved by the same-structure designs for both the CL and BERT pre-training. Also, BERT achieves overall better result than CL. It supports our results and claims in Section \ref{sec:structure} regarding the benefit of using the same model structure.

% \begin{table}[htb]
%     \centering
%     \resizebox{0.6\columnwidth}{!}{
%     \begin{tabular}{c|cc|cc|cc|}
%          &  \multicolumn{2}{c}{\textbf{ML-1M}} & \multicolumn{2}{c}{\textbf{Instacart}} & \multicolumn{2}{c}{\textbf{Amzn Electronics}} \\ \hline
%          & F1 & AUC & F1 & AUC & F1 & AUC \\ \hline
%         CL-LR &  &  &  &  &  &  \\
%         CL-IP &  &  &  &  &  &  \\ \hline
%         BERT-LR &  &  &  &  &  &  \\
%         BERT-IP &  &  &  &  &  &  \\ \hline
%     \end{tabular}
%     }
%     \caption{\footnotesize Experiment results for structure selection.}
%     \label{tab:structure}
% \end{table}



\textbf{Kernel view for OOD performance.} We examine the kernel-based evaluation for OOD performance on item classfication and sequential recommendation tasks. For both tasks, we train the item embeddings in an Item2vec fashion \cite{barkan2016item2vec} using the user interaction data. To obtain pre-trained embeddings with different qualities, we vary the window size and the \#negative samples, i.e. select them from $\{2,3\}$ and $\{1,2,3\}$. We find that within this range, the larger the window size and \#negative samples, the better the pre-trained embeddings. For item classification, we use logistic regression, kernel regression and two-layer MLP as downstream models. Due to the space limitation, we leave the item classification results to the online material (because it is rather straightforward). 
For sequential recommendation, we experiment with \textbf{Dense} layers, \textbf{GRU} as well as the self-attention (\textbf{Attn}) mechanism to aggregate the item embeddings into the sequence embedding, as depicted in the two-tower structure in Figure \ref{fig:online_eval}a. We use the item popularity as a proxy of the exposure distribution for the kernel-based evaluation. Its hyper-parameter $\alpha$ is also selected via the validation set. We use top-10 \textbf{recall}, the overall \textbf{NDCG} and mean reciprocal rank (\textbf{MRR}) as the evaluation metrics. During kernel-based evaluation, we rank the candidates according the score in (\ref{eqn:seq-score}). The relation between the kernel-based evaluation and the models' performances in Figure \ref{fig:OOD}. Since Instacart does not provide sequential information, we focus on the other two datasets. We observe a strong correlation between the kernel-based evaluation, and the actual models' performances, for all the models across the two datasets. They all suggest the effectiveness of the kernel-based evaluation.

\begin{figure}[hbt]
    \centering
    \includegraphics[width=\linewidth]{image/seq-reco-metric.png}
    \caption{\footnotesize Relation between the kernel-based evaluation and the models' performances on the sequential recommendation task.}
    \label{fig:OOD}
\end{figure}


\subsection{Real-world Deployment Analysis}
\label{sec:deployment}

The previous results have provided strong evidence to carry the kernel-based evaluation further to online experiments, which we conduct with \emph{Walmart.com} -- a major e-commerce platform in the U.S. The production scenario is that on the item page, we rank the recall set according to the customers' most recent ten views. We also adopt the two-tower architecture, and handle the other features such as rating, popularity, price range similar to the deep \& wide method \cite{cheng2016wide}. The problem at hand is to find the most desirable pre-trained item embeddings from the three candidates: (1). the item embedding based trained by Doc2vec on the title and description (\textbf{Emb1}), which is currently in production; (2). the item complementary embedding (\textbf{Emb2}) described in \cite{xu2020knowledge}; (3). the knowledge-graph item embedding (\textbf{Emb3}) described in \cite{xu2020product}. 

In the regular offline evaluation, we use each candidate embeddings to retrain the whole model and compute the offline metric. This approach is less efficient because we must tune each model separately to achieve a fair comparison. Also, due to the existence of other features, it is hard to justify only by the offline result whether the differences owe entirely to the embeddings' quality. The proposed kernel-based evaluation is more straightforward and allows fast computation. However, the tradeoff is that we are not entirely confident that the kernel-based evaluation will indeed imply the online performance. Therefore, we conduct both evaluations, and compare them with the online A/B/C test results, as provided in Table \ref{tab:offline_eval} and Figure \ref{fig:online_eval}b.
During evaluations, we find clear distinguishment among the values in the kernel-based evaluation, with \textbf{Emb3}>\textbf{Emb2}>\textbf{Emb1} in both recall and NDCG (Table \ref{tab:offline_eval}). However, the comparisons are almost edge-to-edge for the regular offline evaluation: even though the general pattern is the same as the kernel-based evaluation, the margins are very thin. As we discussed, the existence of other features make the comparison not strictly for the pre-trained embeddings. 
During online testing (Figure \ref{fig:online_eval}), we observe \textbf{Emb3}>\textbf{Emb2}>\textbf{Emb1} in terms of GMV, number of orders, and conversion rate. The deployment result shows that the kernel-based evaluation provides quick and perhaps reliable examinations in terms of the quality of pre-trained embeddings. We do point out that the kernel-based evaluation is not meant to replace other offline evaluations. Instead, it adds to the arsenal a convenient and powerful tool for the practitioners. 


\begin{table}[htb]
    \centering
    \resizebox{\columnwidth}{!}{
    
    \begin{tabular}{c|cc|cc|cc|}
         &  \multicolumn{2}{c}{\textbf{ML-1M}} & \multicolumn{2}{c}{\textbf{Instacart}} & \multicolumn{2}{c}{\textbf{Amzn Electronics}} \\ \hline
         & F1-micro & AUC & F1-micro & AUC & F1-micro & AUC \\ \hline
        CL-LR & 22.89/.70 & 70.25/.90 & 34.5/.52 & 76.3/.77 & 41.25/.41 & 82.44/.60 \\
        CL-IP & 24.50/.65 & 73.46/.88 & 35.92/.48 & 78.05/.71 & 42.46/.38 & 83.97/.56 \\ \hline
        BERT-LR & 30.25/.73 & 77.46/.44 & 38.12/.36 & 80.53/.68 & 46.42/.33 & 86.07/.49 \\
        BERT-IP & 24.67/.58 & 74.03/.56 & 35.95/.40 & 78.21/.71 & 43.29/.36 & 84.70/.52 \\ \hline \hline
    
    \multicolumn{7}{c}{\vspace{0.5cm}} \\
    
         &  \multicolumn{2}{c}{\textbf{Emb1}} & \multicolumn{2}{c}{\textbf{Emb2}} & \multicolumn{2}{c}{\textbf{Emb3}} \\ \hline
         & Hit@5 & NDCG@5 & Hit@5 & NDCG@5 & Hit@5 & NDCG@5 \\ \hline
        Kernel & 9.26 & 4.55 & 11.38 & 5.71 & 14.47 & 6.80 \\
        Regular & 21.02 & 9.86 & 21.68 & 9.94  & 21.74 & 9.92 \\ \hline
    \end{tabular}
    }
    \caption{\footnotesize \text{Upper}: impact of model design for i.i.d downstream task. \textbf{Lower}: the offline evaluations results, using the tranditional evaluation and the proposed kernel-based evaluation. Results are multiplied by 100.}
    \label{tab:offline_eval}
\end{table}

\begin{figure}[hbt]
    \centering
    \includegraphics[width=\linewidth]{image/ind-two-tower.png}
    \caption{\footnotesize (a) The two-tower architecture for sequential recommendation. (b) The online A/B/C testing result with \textbf{Emb1} (\textbf{Control}), \textbf{Emb2} (\textbf{Variation 1}) and \textbf{Emb3} (\textbf{Variation 2}).}
    \label{fig:online_eval}
\end{figure}








==> introduction.tex <==
As deep learning continues to reshape e-commerce machine learning, pre-trained embeddings have become a standard building block in many solutions. Researchers are motivated to design pre-training algorithms for increasingly complex problems \cite{barkan2016item2vec,wang2018billion,xu2020product,vasile2016meta,wan2018representing,xu2020knowledge,zhang2020towards}, and practitioners have made significant progress in training and serving embeddings for industry-scale ML \cite{covington2016deep,huang2020embedding,grbovic2018real}.

The need of using pre-trained embeddings stems from the challenge of dealing with unstructured and sparse features, which are particularly abundant in e-commerce. 
In recent years, embedding-based solutions are dominating sequential recommendation \cite{fang2020deep}, cold-start problem \cite{saveski2014item}, cross-task and cross-domain recommendation \cite{man2017cross}, and even causal recommendation \cite{fei2019end,bonner2018causal}. 
Besides recommendation, pre-trained embeddings also play critical roles e-commerce-specific tasks such as \emph{content understanding}, examples include segmenting or clustering items and users \cite{xu2021theoretical,wan2018representing,jie2021bidding}.
However, the popular usage of pre-trained embedding should not be considered evidence of a warrantied solution. In e-commerce, practical domain issues can drive pre-trained embeddings outside the guarantees provided by the original disciplines \cite{allen2019analogies,arora2016latent}. As a consequence, the use of pre-trained embeddings may further complicate the black-box nature of deep learning solutions, and their effectiveness are ultimately left to empirical judgement rather than rigorous understanding.

We particularly study the optimization and generalization properties of pre-trained embeddings for recommendation and content understanding, which are arguable the two most important tasks in e-commerce ML.
We will explain later how our investigations relate to the practical challenges in the model design, training, and evaluation. As pre-trained embedding is holding dominating popularity in both academia and industry, we aim to establish principled guidelines and understandings that contribute to both the theoretical research and real-world application. 
To provide readers with some insight, consider the following scenarios that are common to real-world e-commerce ML. 

\begin{example}
\textup{
Suppose there is a downstream model in place which consumes pre-trained embeddings. Imagine that new data becomes available and the embeddings are re-trained: \\
\textbf{Q1}: Can we keep the downstream model as-is, or do we also retrain it from scratch? \\
\textbf{Q2}: If the new embeddings show better performances in offline nearest-neighbor search, are they guaranteed to improve the downstream task?
}
\end{example}

\begin{example}
\textup{
When a new task is assigned and a downstream model is proposed: \\
\textbf{Q3}: Can we reuse the existing embeddings, or use another pre-training procedure that is compatible with the proposed model? \\
\textbf{Q4}: Since the pre-training data is not collected from the new task's environment, how do we predict the out-of-distribution (OOD) performance of pre-trained embeddings?
}
\end{example}


% These questions are essential for e-commerce ML, for instance, retraining the entire model from scratch is often costly, and mistakenly launching A/B testings can hurt the revenue.
Clearly, not knowing the working mechanisms of pre-trained embeddings is a major cause of the questions: \textbf{Q1} asks about the robustness of pre-training, \textbf{Q2} and \textbf{Q3} concerns the impact of model design on the downstream generalization, and \textbf{Q4} requires understanding OOD performance of pre-trained embedding. 
% These topics have received relatively less attention since they concerns only a particular subset of the general machine learning theory. However, they are critical for the decision making in real-world recommender systems, and it is therefore the goal of this paper to fill in the gaps.

Unfortunately, the mechanisms behind pre-trained embeddings are often more complicated then we might expect. In particular, we point out the problem of using the popular \emph{Contrastive Learning} (CL) to pre-train item embeddings. The pre-trained embeddings are then used for downstream classification tasks, a procedure that is fairly standard in recent literature \cite{barkan2016item2vec,wan2018representing,xu2020product,xu2020knowledge,xu2021theoretical,grbovic2015commerce,vasile2016meta}. 

As a briefly introduction, CL enforces the inner product of "semantically similar" item representations to be larger than that of the randomly sampled negative pairs. For now, we use $\Ical = \big\{i_1,\ldots,i_p\big\}$ to denote the set of items. For an item $i$, we denote the positive pair as $\big(i,i^+\big)$ and the negative pair as $\big(i,i^-\big)$. The (hidden) representation of an item is a function: $\phi: \Ical \to \Rbb^d$, which can be parameterized by any neural network. In this paper, we use the notion of (hidden) representation and embedding interchangeably, but keep in mind that they can be further parameterized by other underlying models. 

Typically, CL optimizes the representations by minimizing the objective function:
\[
\Ebb \Big[ -\log \frac{e^{\phi(i)^{\intercal}\phi(i^+)}}{e^{\phi(i)^{\intercal}\phi(i^+)} + e^{\phi(i)^{\intercal}\phi(i^-)}} \Big].
\]
% It may occur to certain readers that the objective of CL coincides with many pariwise loss or ranking functions from the information retrieval literature \cite{pasumarthi2019tf}. Here, we use CL as a general reference to this type of objective functions.

Although the inner product between representations often produces meaningful similarity scores, the \emph{exact value} on each dimension of the embeddings are less examined. However, most downstream tasks, including item classification, consume embeddings as numerical vectors rather than using their inner products. 
This usage is potentially problematic, because the algebraic formulation of inner product may induce \textbf{spurious dimensions} whose values can change without affecting the outcome. 
Furthermore, the random negative sampling may lead to $\big(i,i^-\big)$ pairs who belong to the same class in downstream classification, causing \textbf{extra variance} in the embedding vectors. We illustrate both phenomenons in the following example.

\begin{example} [\textbf{Spurious dimensions}]
\label{example:spurious}
Suppose the negative pair $(i_1,i_2)$ can be perfectly classified on the $y$ direction (see Figure \ref{fig:illustration}a). It means $(i_1,i_2)$ is a perfect negative pair.
The representation hypothesis $\Hcal_1$ projects $i_1$ and $i_2$ to the affine subspace (the green line) and leads to the representations $\phi(i_1)$ and $\phi(i_2)$ which can be perfectly classified. 

On the other hand, the representation hypothesis $\Hcal_2$ (the red line) projects $i_1$ and $i_2$ to the $x$ direction, where $\phi(i_1)$ and $\phi(i_2)$ become inseparable. 
In this example, the horizontal direction is the spurious direction, while the vertical direction is discriminative. Unfortunately, the \emph{absolute value} of the inner product on the spurious direction (given by $\big[\phi(i_1)\big]_x \times \big[\phi(i_2)\big]_x$) dominates that of the discriminative direction (given by $\big[\phi(i_1)\big]_y \times \big[\phi(i_2)\big]_y$). Therefore, the CL algorithm will falsely favor $\Hcal_2$.
\end{example}

\begin{figure}[hbt]
    \centering
    \includegraphics[width=\linewidth]{image/illustration.png}
    \caption{Sketched visual illustrations for Example \ref{example:spurious} and \ref{example:imperfect}. The \emph{colored lines} represent the hypothesis spaces, and the \emph{dashed lines} project the data points to the hypothesis spaces.}
    \label{fig:illustration}
    \vspace{-0.2cm}
\end{figure}

\begin{example}[\textbf{Imperfect negative sampling}]
\label{example:imperfect}
Suppose for an item $i$ that another item $i_1$ appears both in the positive pair $\big(i,i_1^+\big)$ according to the observed data, as well as in the negative pair $\big(i,i_1^-\big)$ because the negative sampling is completely random. This case is illustrated in Figure \ref{fig:illustration}b, where we only plot $i_1^+$ and $i_1^-$ for clarity, since the location of $i$ will not matter in our analysis. 

Under the same representation hypothesis $\Hcal_1$ from the previous example, for item $i_1$, the projections for $\phi(i_1^+)$ and $\phi(i_1^+)$ will be different since. $i_1$ appears in both the positive and negative pairs. As a result, the expected representation of $\phi(i_1)$ will depend on how likely $(i,i_1^-)$ is sampled.
\end{example}

\textbf{Important implications:} Example \ref{example:spurious} reveals the possibility that CL may prioritizing the hypothesis that minimizes the inner product on the spurious dimensions, rather than focusing entirely on the discriminative dimensions. 
The negative sampling schema of CL, as we discussed in Example \ref{example:imperfect}, can also brings uncertainty to the learnt embeddings. 

Both examples suggest that CL-based pre-training experience fundamental optimization issues rooted in the algorithmic design. In Section \ref{sec:preliminary}, we rigorously discuss how it leads the hardness of learning by using pre-trained embeddings as numerical feature vectors. To briefly summarize, our work contributes to:
\begin{itemize}[leftmargin=*]
    \item revealing the hidden technical debts of pre-training embeddings that are less mentioned in the literature;
    \item investigating how modelling assumption and algorithmic design affect the interplay between pre-training to downstream tasks;
    \item establishing a principled kernel view that reveals the expressivity and provides practical OOD evaluations of pre-trained embeddings for e-commerce ML.
\end{itemize}
All our claims and explanations are illustrated by experiments on benchmark datasets. Readers less familiar with learning-theoretical arguments can safely skip the math details and focus on our illustrative experiments and their implications. 
Domain experts who seek deeper understanding may benefit further from our theoretical results and the subsequent remarks.

% The paper is organized as follow. In Section \ref{sec:preliminary}, we first describe the basic settings of our experiments that serve to justify the major claims and theoretical results in our paper. We also introduce the preliminaries in Section \ref{sec:preliminary}. We then investigate the generalization performance of different pre-training design in Section \ref{sec:structure}, and establish the kernel view in Section \ref{sec:kernel}. In Section \ref{sec:related}, we discuss how our results connect to, explain, and provide theoretical justifications for several existing topics. 

% With all the discussions rooted in practice, we hope our work promotes the understanding of pre-trained embeddings for both researchers and practitioners in the community.


==> rebuttal.tex <==
We thank all reviewers for the valuable comments and feedback on our manuscript.
As is suggested by the reviewers, our paper represents a scarce but important type of work, which provides rigorous justifications and understandings toward domain practices and phenomenons. 
Our paper provides a demonstration that ML paper in this field, while often deemed as empirical and result-centric, can also possess and benefit from a decent amount of rigorousness. 
In what follows, we address the individual concerns from the reviewers.

===================================
To R1:

We thank the reviewer for recognizing the novelty and importance of our work. We do apologize for making explicit an institution's name, but we tried to follow the Call for Paper instruction listed on the conference's webpage: "...instead of saying that "we analyzed the logs of a major search engine", the authors may name the search engine in question. The reviewers will be informed that naming organizations in papers do not necessarily imply that the authors are currently affiliated..." 

We sincerely hope it did cause too much confusion, and we thank the reviewer again for reviewing our manuscript.

===================================
To R2:

We thank the reviewer for the careful reading and valuable advice. We apologize for the typos, and we believe there are a few misconceptions that, once clarified, will help the reviewer better understand the contribution of our work.

To Q1. We have honestly considered adopting the writing style of [1]; however, the complexity of our topics and the depth of our theoretical insights clearly superseded that of [1]. To ensure that even entry-level readers can understand the key takeaways, we corroborate all the theoretical results with comprehensive explanations and empirical experiments. Just because our presentation does not follow traditional DM/IR literature, it does not mean researchers and practitioners cannot benefit from our work. In fact, the reviewer has also mentioned that our results and insights are helpful to both academia and industry. Also, there might be one misconception from the reviewer: the primary focus of our work should be ML rather than DM/IR. In particular, recommendation is only one of the ML tasks of interest, and pre-trained embeddings are often employed in multiple scenarios in e-commerce. It might be inappropriate to perceive our manuscript as a DM/IR work with all due respect.

To Q2. The reviewer raised a great question. In short, our result applies to ALL models that use the inner product to measure similarity and use the negative-sampling-based optimization. With that said, the final presentation can come from the last hidden layer of any deep learning model, e.g. BERT, as we have illustrated in our experiments. We use item2vec to elaborate our results simply because it is straightforward; however, our results hold under a much broader spectrum of models. The in-batch softmax should not change our arguments as long as each batch are i.i.d. Sequential pre-training (e.g. using the two-tower architecture) also follows our results as long as the inner product and negative-sampling-based optimization are employed. We will make these points clear in the next revision, and we believe the generalization ability of our results should not be a major concern.

===================================
To R3:

We appreciate the reviewer for checking our manuscript. However, we are baffled by the reviewer's comments, as many of them reflect a severe lack of understanding of industrial ML in general. If so, we are afraid the reviewer's misconceptions have led to inappropriate and unfair evaluations of our work, which we point out as below:

To Q1. We have clearly outlined where we answer all the optimization, robustness, and generalization questions. It seems that only Reviewer3  ran into problems grasping the takeaways of our work. We understand the reviewer may not have enough time to review our manuscript, but drawing such a conclusion based on the reviewer's own misreading seems irresponsible and unprofessional. 

To Q2. Pre-trained embeddings is an indispensable part of all large-scale real-world ML systems, and e-commerce is no exception. We are NOT aware of any literature that claims using end-to-end DL training on billions of entities and still actively serving real-world ML systems. The reviewer might have come across demonstrations conducted offline, but running an ML system online is a whole different story. We hope the reviewer can provide concrete evidence to ground the accusation.

To Q3. We are very confused by this question because our work EXACTLY tries to address machine learning problems. The questions we raised are grounded in industrial production and point to particular ML problems, e.g. robustness of optimization with negative sampling, OOD generalization. They are critical research questions, particularly for e-commerce, considering how ML systems are designed in this field. Other domains may also benefit from our results, but it seems the reviewer considers having a broader impact as a drawback of our work, which seems unreasonable. 

==> rebuttal_www.tex <==
Dear Meta Reviewer:

We would first like to thank all reviewers for their time and efforts. But with all due respect, we must point out the many factual errors in the reviewers' comments, especially those from REVIEWER 2 and REVIEWER 3.

Factual errors in REVIEWER 2's comments on our weakness:

For W1. The reviewer misreads our experiment setting: the sampling-negatives-from-other-class experiment is only meant for controlling confounding factors for illustration in Section 2, and it has nothing to do with our following analysis and proposed approach.

For W2. As our title shows, the scope of our paper is e-commerce ML. Why does the reviewer wants us to experiment with news recommendation? This is by no means a weakness of our paper but a mistake of the reviewer. 

Finally, the reviewer criticizes us for not using e-commerce specific properties in our experiments, which is absurdly wrong. In our online experiments, all treatment variants clearly use e-commerce product properties (otherwise the A/B/C testing could have never been approved). It appears the reviewer did not read through our experiments carefully and responsibly. 

Factual Errors in REVIEWER 3's comments on our weakness:

For W1: We made it very clear in our paper that the perturbation in Figure 1 is not an artefact of seed choice but the stochastic nature of random initialization. The "phi(x)+epsilon" notion is a simplified elaboration on the lingering post-optimization stochastic effects.

For W2: The reviewer criticize us for not comparing with existing indicators. To our knowledge, there are no readily available indicators (on the predictability of pre-trained embeddings) to compare with, and the reviewer does not responsibly provide any references or explanations. 

For W3: We have no idea why the reviewer would consider deferring the lengthy technical proofs to appendix as a weakness of our presentation. This is customary for all major conferences, and the reviewer seems to be nitpicking.

For W4: The reviewer's comment is far from correct. Any educated scholar would agree that online experiment carries less bias than offline evaluation. Examining with the right metrics and eliminating confounding factors is exactly what online experiments are for. 

Finally, while criticizing us for wasting space deriving the setups, the reviewer asks us to add the proofs back to the paper, which is clearly contradictory. We hope the Meta Reviewer can tell the quality of REVIEWER 3's comments from all these factual errors and conflicting comment.

As authors, we understand that less qualified reviews may slip through even for The Web Conference, and we are obligated to point them out for the Meta Reviewer. All the evidence above shows that the reviews from REVIEWER 2 and REVIEWER 3 do not constitute any fair evaluation of our work. We merely hope the Meta Reviewer can look into the above evidence and give a fair evaluation that any hard work deserves.

Best regards, 
Authors

